Bayesian Probabilistic Numerical Methods

The emergent field of probabilistic numerics has thus far lacked clear statistical principals. This paper establishes Bayesian probabilistic numerical methods as those which can be cast as solutions to certain inverse problems within the Bayesian framework. This allows us to establish general conditions under which Bayesian probabilistic numerical methods are well-defined, encompassing both non-linear and non-Gaussian models. For general computation, a numerical approximation scheme is proposed and its asymptotic convergence established. The theoretical development is then extended to pipelines of computation, wherein probabilistic numerical methods are composed to solve more challenging numerical tasks. The contribution highlights an important research frontier at the interface of numerical analysis and uncertainty quantification, with a challenging industrial application presented.

==> bayes_mean_proof.tex <==
%!TEX root=./pn_foundations.tex
We seek $h(a) \in \mathcal{Q}$ minimising
\begin{equation*}
	\expected[\norm{Q(x) - h(a)}^2] ,
\end{equation*}
where we have suppressed the subscript on $\norm{\cdot}_\mathcal{Q}$.
By the properties of conditional expectations, conditional upon $A_M x = a$ this is equivalent to minimising
\begin{equation*}
	\expected\left[ \expected[ \norm{Q(x) - h(a)}^2 | A_M x = a]\right] .
\end{equation*}
Now
\begin{align*}
	\norm{Q(x) - h(a)}_Q^2 &= \norm{Q(x)}^2 - 2 \inner{Q(x), h(a)} + \norm{h(a)}^2 \\
%	&= \norm{Q(x)}^2 - 2 \inner{Q(x), h(a)} + \inner{h(a), h(a)} \\
	&= \norm{Q(x)}^2 + \inner{Q(x) - h(a), h(a)}
\end{align*}
by properties of inner products.
Only the second term depends upon $h(a)$, so we must minimise
\begin{equation*}
	\expected\left[\inner{Q(x) - h(a), h(a)} | A_M x = a \right]
		= \inner{\expected\left[Q(x) | A_M x = a\right] - h(a), h(a)} ,
\end{equation*}
which is minimised by $h(a) = \expected(Q(x) | A_M x = a)$.
This is precisely $\expected(Q_\# \pi_M(a))$, which completes the proof.

==> experiment_manifold.tex <==
%!TEX root = ./pn_foundations.tex

In this section we illustrate the idea of Section \ref{sec:rcp_smc} by constructing a sampler for the disintegration of a uniform distribution $U([-1,1]^2)$ onto an embedded circular manifold, centered on the origin with a radius of $0.8$.
It is convenient to consider this restriction in polar coordinates $(r, \theta)$, where $r=\sqrt{x_1^2 + x_2^2}$ and $\theta = \tan^{-1}(x_2/x_2)$; then the manifold is given by the curve $r=0.8$, $\theta\in[-\pi, \pi]$. 

To associate with the notation of the rest of the paper, the domain is given by $\mathcal{X} = [0,1]^2$ while $\mathcal{A} = \reals$;
$\nu \sim U([-1, 1]^2)$ and the operator $A \colon X\to \mathcal{A}_M$ is given by $A_M\bm{x} = \sqrt{x_1^2 + x_2^2}$.

Since this is a finite-dimensional problem, the information-complexity difficulty with having only finite information about a high- or infinite-dimensional object is no longer present;
here $Y$ is one-dimensional.
Thus $A_M\equiv A$ and our ``data'' $a$ is simply the value $a = 0.8$.
Similarly, progressively smaller balls $B_\delta(a)$ translate to intervals of the real line about $0.8$.
This is illustrated in Figure \ref{fig:manifold_example}.

The experiment is conducted for an ensemble of $100,000$ particles, with $\set{\delta_i}$ for $i=1,\dots,20$ taken to be equally spaced between $1$ and $10^-8$ in log-space.
For each $\delta_i$ our transition kernel $K_i(x_i^j)$ is Gaussian with mean $x_i^j$ and variance $2\delta_i$, which is found empirically to give a good acceptance probability for all $\delta_i$.

An illustration of the posterior distribution for the final $\delta_{20} = 10^{-8}$ in Euclidean space is given in Figure \ref{fig:manifold_samples_euclidean}.
The target manifold is 1-dimensional, and we expect the distribution over $r$ to be approximately a constant, while the distribution over $\theta$ should be approximately uniform.
The posterior distribution for $\delta_{20}$ in polar coordinates is given in Figure \ref{fig:manifold_samples_polar}.
As expected, we see that the distribution of the radial component is approximately uniform over an interval of $0.8 \pm 10^{-8}$ while the angular component is uniform over $[-\pi, \pi]$.

\begin{figure}
	\centering
	\includegraphics[width=0.5\textwidth]{figures/SMC_procedure.pdf}
	\caption{An illustration of the SMC procedure from Section \ref{sec:example_manifold}, with $\delta=0.1$ and 40 particles. Green crosses indicate particles which satisfy the ball condition and will be accepted; black crosses are those which will be rejected, and thus be sampled uniformly from the accepted particles.} \label{fig:manifold_example}
\end{figure}
\begin{figure}
	\begin{subfigure}{\textwidth}
	\centering
	\includegraphics[width=0.4\textwidth]{figures/manifold_samples_euclid.pdf}
	\caption{Euclidean Space} \label{fig:manifold_samples_euclidean}
	\end{subfigure}
	\begin{subfigure}{\textwidth}
		\includegraphics[width=\textwidth]{figures/manifold_samples_r_theta.pdf}
		\caption{Polar coordinates}
		\label{fig:manifold_samples_polar}
	\end{subfigure}
	\caption{Posterior distribution for the disintegration of measure problem.}
\end{figure}


==> smc_error_proof.tex <==
%!TEX root=./pn_foundations.tex
We will apply Theorem 7.4.4 of \cite{DelMoral:2004fe}.
This requires several assumptions, which are related to Assumption.~\ref{assumption:reachable} and Assumption~\ref{assumption:composition}.
We first associate notation.
To this end, Del Moral's transition kernel $M$ is denoted $K$ in this work.
The potentials $G$ are indicator functions; $G_i(x) = \indicator(x \in X_a^{\delta_i})$.
$E_i$ in Del Moral denotes the set of points on which each potential is defined;
in our setting this is simply $\mathcal{X}$, for all $i$. $\hat{E}_i$  denotes those points for which the potential at level $i$ is nonzero, which corresponds to our $X_a^{\delta_i}$.
We also note that while Del Moral requires $i \in \mathbb{N}$, in our setting we have a finite temperature schedule and so $0 \leq i \leq m$.

% this reparameterization occurs on Del Moral p65
Since our potentials are vanishing, we must first consider the reparameterization indicated in Del Moral's Section 7.2.2. To this end let 
\begin{align*}
	\hat{G}_i &= M_{i+1}(G_{i+1}) \\
	\hat{G}(x) &= \int_{\mathcal{X}} G_{i+1}(y) M_{i+1}(x, \wrt y) \\
	&= \int_{X_a^{\delta_{i+1}}} M_{i+1}(x, \wrt y) \\
	&= M_{i+1}(x, X_a^{\delta_{i+1}})
\end{align*}
and apply all assumptions to this adjusted potential $\hat{G}_i$.
The adjusted transition $\hat{M}_i$ is simply the restriction of the transition kernel $M_i$ to the set $X_a^{\delta_{i+1}}$ in our setting.
Since we have assumed that the $K_i$ target $\pi_M^{\delta_i}(a)$ the adjustment demanded has no effect, so that $M_i \equiv \hat{M}_i$; thus we will use $M_i$ directly throughout. 
Theorem 7.4.4 then depends upon the following assumptions in \cite{DelMoral:2004fe}:

\begin{itemize}
\item {\it Assumption $(G)$ (p115)}

This states that, for any $x_n \in E_n$
\begin{equation*}
	G_n(x_n) \geq \epsilon_n(G) G_n(y_n)
\end{equation*}
Our $\hat{G}_n(x)$ is simply $K_{i+1}(x, X_a^{\delta_{i+1}})$.
Since this is bounded above by 1, we need only confirm that $K_{i+1}(x, X_a^{\delta_{i+1}})$ is bounded away from zero, for any $x \in X_a^{\delta_i}$.
This is true by Assumption~\ref{assumption:reachable}.

\item {\it Assumption $(M)_m$ (p116)}

We take $m=1$, so that this is a statement about the transition kernel itself rather than chained together versions thereof. Thus we require that
\begin{equation}
	\label{eq:del_moral_assumption_M}
	M_{i+1}(x_p, \cdot) \geq \epsilon_p(M) M_{i+1}(y_p, \cdot)
\end{equation}
for all $x_p, y_p \in X_a^{\delta_i}$.
The notation $M_{i+1}(x_p, \cdot)$ must be interpreted as a density with respect to some reference measure;
the natural measure for our setting is the prior.
Thus we may re-express Eq.~\eqref{eq:del_moral_assumption_M} as
\begin{equation*}
	\frac{
		M_{i+1}(x_p, \cdot)
	}{
		M_{i+1}(y_p, \cdot)
	} \geq \epsilon_p(M)
\end{equation*}
and recongnise the ratio of densities on the left as the \radonnikodym derivative $\frac{\wrt K_{i+1}(x_p, \cdot)}{\wrt K_{i+1}(y_p, \cdot)}$ since, by Assumption~\ref{assumption:composition}, $K_{i+1}(x_p, \cdot) \ll K_{i+1}(y_p, \cdot)$ for any $x_p, y_p \in X_a^{\delta_i}$.
Thus the required inequality is guaranteed by Assumption~\ref{assumption:composition}.


\item {\it Assumption $\mathcal{A}$ (p220)}

Since we have $\hat{E}_0 = \mathcal{X}$, $\eta_0 = \pi$ and so this is a requirement that $\pi(\mathcal{X}) > 0$, guaranteed by the fact that $\pi$ is a distribution defined on $\mathcal{X}$.
The requirement that $M_{i+1}(x_i,\hat{E}_{i+1}) > 0$ is a weaker version of Assumption $(G)$, above, in the present setting.

\end{itemize}

For any $f\in L^\infty_\pi(\mathcal{X})$, let $\textrm{Osc(f)} = \esssup_{x, y \in \mathcal{X}} \abs{f(x) - f(y)}$. Clearly $\textrm{Osc}(f) = 0 \iff f = c$, $\pi-a.s.$, for some constant $c$.
Since this is a trivial edge-case we will assume $\textrm{Osc}(f) > 0$ in what follows.

Let $\textrm{Osc}_1(\mathcal{X})$ denote those $f$ with $\textrm{Osc}(f) \leq 1$. Then clearly, for any $f \in L^\infty_\pi$,
\begin{equation*}
	\hat{f}\defeq \frac{f}{\textrm{Osc}(f)} \in \textrm{Osc}_1(\mathcal{X}) \;.
\end{equation*}

With the validity of the requisite assumptions established we may apply Del Moral's Theorem 7.4.4 to our setting.
This states that, for any $0 \leq i \leq n$, $p\geq 1$ and any $f_i \in \textrm{Osc}_1(\mathcal{X})$, we have
\begin{equation*}
	\sqrt{N} \mathbb{E}\left(\abs{ 
		\left[ \pi_M^{\delta_i, N}(a) - \pi_M^{\delta_i}(a)\right](f_i)
	}^p\right)^{\frac{1}{p}} 
	\leq 2 d(p)^\frac{1}{p} \sum_{q=0}^i r_{q,i} \beta(P_{q,i})
\end{equation*}
where $r_{q,i}$ and $\beta(P_{q,i})$ are each regularity parameters for the potentials and the transition kernels respectively, introduced in Del Moral's Eq.~7.3, and $d(p)$ is given by
\begin{equation*}
	d(2p) = (2p)_p 2^{-p} \qquad d(2p-1) = \frac{(2p-1)_p}{\sqrt{p-1/2}} 2^{-(p - 1/2)} \;.
\end{equation*}
Here $(n)_p = \frac{n!}{(n-p)!}$.

Our Theorem \ref{thm:smc_error} follows directly by taking $p=2$, taking $f \in L_\pi^\infty(\mathcal{X})$ and applying the result above to $\hat{f}$.
Let
\begin{equation*}
	D(p) = 2 d(p)^\frac{1}{p} \sum_{q=0}^n r_{q,n} \beta(P_{q,n}) \;.
\end{equation*}
and note that since $\textrm{Osc}(f)$ is constant it can be removed from the expectation to give
\begin{equation*}
	\mathbb{E}\left(\abs{ 
		\left[ \pi_M^{\delta_i, N}(a) - \pi_M^{\delta_i}(a)\right](f_i)
	}^p\right)^{\frac{1}{p}} 
	\leq \frac{D(p) \; \textrm{Osc}(f)}{\sqrt{N}} \;.
\end{equation*}
Finally note that $\textrm{Osc}(f) \leq 2\norm{f}_\infty$; replacing $\textrm{Osc}(f)$ with this more familiar norm and letting $C = 2D$ gives the required result.

